Game Theory in Distributed Systems Security: Foundations, Challenges, and Future Directions

Many of our critical infrastructure systems and personal computing systems have a distributed computing systems structure. The incentives to attack them have been growing rapidly as has their attack surface due to increasing levels of connectedness. Therefore, we feel it is time to bring in rigorous reasoning to secure such systems. The distributed system security and the game theory technical communities can come together to effectively address this challenge. In this article, we lay out the foundations from each that we can build upon to achieve our goals. Next, we describe a set of research challenges for the community, organized into three categories -- analytical, systems, and integration challenges, each with "short term" time horizon (2-3 years) and "long term" (5-10 years) items. This article was conceived of through a community discussion at the 2022 NSF SaTC PI meeting.

==> header.tex <==
\usepackage{fullpage,url,wrapfig}
\usepackage[font={bf,it,footnotesize},labelsep=colon,justification=centering]{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{color}
\usepackage{amsmath}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{fullpage}
\usepackage{bm}
% \usepackage{enumitem} % left lists.
\usepackage{xspace}
\usepackage{comment}
%\pagestyle{plain}

%\usepackage[hidelinks,colorlinks=false]{hyperref} % For autorefs and hyperlinks
\usepackage{cleveref}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{algorithm} % For algorithm floats, must be after hyperref
\usepackage{algorithmic} % ICML suggested packages
\usepackage{mathtools} % Automatically loads amsmath
\usepackage{amsthm, amssymb, amscd, amsfonts} % Other AMS packages
\usepackage{thmtools}
\usepackage{thm-restate} % So that theorems can be restated in appendix with proofs
\usepackage{multirow}
\usepackage{multicol}
\usepackage{verbatim}
\usepackage{soul}

% General-purpose macros
\renewcommand{\thepage}{\arabic{page}}
%\newcommand{\Section}[1]{\section*{#1} \setcounter{page}{1}}

\newcommand{\eg}{{e.g.,}\xspace}
\newcommand{\ie}{{i.e.,}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\chop}[1]{}
\newcommand{\choprev}[1]{\st{#1}} % chops for the second revision

% ApproxDet macros
\newcommand{\iconsupport}{\includegraphics[width=0.17in]{Figures/icon_support.png}}
\newcommand{\iconpartsupport}{\includegraphics[width=0.17in]{Figures/icon_part_support.png}}
\newcommand{\iconnotsupport}{\includegraphics[width=0.17in]{Figures/icon_not_support.png}}

% E2C macros
\newif\ifdraft
\newif\iffull
\newif\ifsubmission

\draftfalse
\fullfalse
\submissiontrue

\def\coolname{E2C\xspace}
\def\protocol{E2C\xspace}

% \newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
% \newtheorem{definition}{Definition}

\def\adv{\ensuremath{\mathcal{A}}\xspace}

% Helper Macros
\newcommand{\sizeof}[1]{\ensuremath{\vert #1 \vert}\xspace}
% \renew
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}\xspace}
\newcommand{\p}[1]{\left(#1\right)}
\newcommand{\pd}[2]{\dfrac{\partial #1}{\partial #2}}

% Communication Primitives
\newcommand{\send}[1]{\ensuremath{\mathsf{send}\p{#1}}}
\newcommand{\sendAll}[1]{\ensuremath{\mathsf{sendAll}\p{#1}}}
\newcommand{\recv}[1]{\ensuremath{\mathsf{recv}\p{#1}}}
\newcommand{\recvAll}[1]{\ensuremath{\mathsf{recvAll}\p{#1}}\xspace}

% Cryptographic primitives
\newcommand{\MAC}[1]{\ensuremath{\mathsf{MAC}\p{#1}}}
\newcommand{\sign}[1]{\ensuremath{\mathsf{Sign}\p{#1}}}
\newcommand{\vrfy}[1]{\ensuremath{\mathsf{Verify}\p{#1}}}

% Graph Properties
\def\K{\ensuremath{k}\xspace}
\def\din{\ensuremath{d_{in}}\xspace}
\def\dout{\ensuremath{d_{out}}\xspace}
\def\kcast{\K-cast\xspace}
\def\kcasts{\K-casts\xspace}
\def\pp{\ensuremath{\mathsf{pp}}\xspace}
\def\h{\ensuremath{\mathcal{H}}\xspace}
\def\V{\ensuremath{\mathcal{N}}\xspace}
\def\E{\ensuremath{\mathcal{E}}\xspace}
\def\pk{\ensuremath{\mathsf{pk}}\xspace}
\iffull
\def\parsepp{\ensuremath{\pp := \p{\h,f,\delay}}\xspace}
\else 
\def\parsepp{\ensuremath{\p{\h,f,\delay}}\xspace}
\fi
\def\parsehgraph{\ensuremath{\h := \p{\V, \E}}\xspace}
\def\parseV{\ensuremath{\V = \set{\node_1,\dots , \node_n}}\xspace}
\def\Nd{\ensuremath{\mathtt{neigh}}\xspace}
\def\sendNd{\ensuremath{\mathtt{send}}\xspace}
\def\recvNd{\ensuremath{\mathtt{recv}}\xspace}
\def\delay{\ensuremath{\Delta_{\h}}\xspace}

% Graph Helper Commands
\def\node{\ensuremath{p}\xspace}
\newcommand{\nodei}[1]{\ensuremath{\node_{#1}}\xspace}
\def\nodes{\ensuremath{\V}\xspace}
\newcommand{\parseVn}[1]{\ensuremath{\V= \set{\node_1,\dots , \node_{#1}}}\xspace}
\newcommand{\parsePK}[1]{\ensuremath{\pk = \set{ pk^{#1}_1,\dots , pk^{#1}_n}}\xspace}
\newcommand{\hedge}[2]{\ensuremath{\set{\node_{#1},\left\{#2 \right\}}}\xspace}
\newcommand{\sedge}[1]{\ensuremath{S\p{ #1 }}\xspace}
\newcommand{\redge}[1]{\ensuremath{R\p{ \set{#1} }}\xspace}
\newcommand{\parsesedge}[2]{\ensuremath{S\p{ #1 } = \set{ #2 } }\xspace}
\newcommand{\parseredge}[2]{\ensuremath{R\p{ #1 } = \set{ #2 } }\xspace}

% Blocks
\def\block{\ensuremath{B}\xspace}
\def\defaultblock{\ensuremath{\blocki{m}}\xspace}
\newcommand{\blocki}[1]{\ensuremath{\block_{#1}}\xspace}
\def\altblock{\ensuremath{B^{\star}}\xspace}
\def\altdefaultblock{\ensuremath{\altblocki{m}}\xspace}
\newcommand{\altblocki}[1]{\ensuremath{\altblock_{#1}}\xspace}
\def\blkcontent{\ensuremath{b}\xspace}
\def\defaultblkcontent{\ensuremath{\blkcontent_{m}}\xspace}
\def\hashptr{\ensuremath{h}\xspace}
\def\defaulthashptr{\ensuremath{\hashptr_{m-1}}\xspace}
\def\parseBk{\ensuremath{\msg{\defaultblkcontent,\defaulthashptr}}\xspace}

% Some constants
\def\IC{Interactive Consistency\xspace}
\def\ICabbr{IC\xspace}
% \def\Tone{Tier~1\xspace}
% \def\Ttwo{Tier~2\xspace}
\def\connectivityresult{\ensuremath{\min\limits_{\nodei{i}\in\nodes} \p{ \dout\p{\nodei{i}},  \din\p{\nodei{i}}  }}\xspace}
\def\hypergraphresult{\ensuremath{\K\cdot\min\p{\din , \dout}}\xspace}
\def\result{\ensuremath{f < \hypergraphresult}\xspace}
\def\smrResult{\ensuremath{f < \min\p{\min\p{\din , \dout} + \K - 1,\tfrac{n}{2}}}\xspace}
\def\faulty{faulty\xspace}
\def\device{\texttt{STM32F407VG}}
\def\opto{\ensuremath{\psi^{\star}}\xspace}
\def\optt{\ensuremath{\psi}\xspace}
\def\optst{\ensuremath{\psi^{Baseline}}\xspace}
\def\opt{\ensuremath{\psi^{\protocol}}\xspace}
\def\nuf{\ensuremath{\nu_f}\xspace}
\def\sigsign{\ensuremath{\sigma_S}\xspace}
\def\sigvrfy{\ensuremath{\sigma_V}\xspace}
\def\sigm{\ensuremath{\sigma_m}\xspace}
\def\macvrfy{\ensuremath{\mu_V}\xspace}
\def\macsign{\ensuremath{\mu_S}\xspace}
\def\tonesend{\ensuremath{T^1_S}\xspace}
\def\ttwosend{\ensuremath{T^2_S}\xspace}
\def\tonerecv{\ensuremath{T^1_R}\xspace}
\def\ttworecv{\ensuremath{T^2_R}\xspace}

% Message types
\def\msgbuf{\ensuremath{\mathsf{msg}}\xspace}
\def\blame{\ensuremath{\mathsf{blame}}\xspace}
\newcommand{\msg}[1]{\ensuremath{\left\langle #1 \right\rangle}\xspace}
\def\propose{\ensuremath{\msg{\mathsf{propose},B_{m},v}}\xspace}
\def\blameMsg{\ensuremath{\msg{\blame,v}}\xspace}
\def\ext{\ensuremath{\mathsf{ext}}\xspace}
\def\commitTimer{\ensuremath{\mathsf{commit\_timer}}\xspace}
\newcommand{\commitTimerof}[1]{\ensuremath{\commitTimer_{#1}}\xspace}
\def\vote{\ensuremath{\mathsf{vote}}\xspace}
\newcommand{\signedmsgc}[2]{\ensuremath{m^{#1}_{#2}, \sigma^{#1}_{#2}}\xspace}
\newcommand{\signedmsg}[2]{\ensuremath{\left\langle \signedmsgc{#1}{#2}
\right\rangle}\xspace}
\def\lockBlock{\ensuremath{B_{lck}}\xspace}
\def\blamecert{\ensuremath{\mathcal{C}\p{\blame,v}}\xspace}
\def\lastcomblk{\ensuremath{\block_{com}}\xspace}
\def\newviewblk{\ensuremath{\block_{nv}}\xspace}
\def\changeview{\ensuremath{\msg{\mathsf{Change-View},\lockBlock,\lastcomblk}}\xspace}
\def\voteMsg{\ensuremath{{\msg{\vote,\lockBlock}_j}}\xspace}
\def\voteMsgnonblk{\ensuremath{\msg{\msg{\vote,v,\lockBlock}_j,
\msg{\vote,v,\lastcomblk}_j}}\xspace}
\def\valnewleaderMsg{\ensuremath{\msg{\mathsf{validate, v+1}}_j}\xspace}
\def\altvoteMsgnonblk{\ensuremath{\msg{\msg{\vote,v,\lockBlock^{\star}}_i,
\msg{\vote,v,\lastcomblk^{\star}}_i}}\xspace}

% Colors
\definecolor{rubine}{cmyk}{0, 0.7808, 0.4429, 0.1412}

% Comment Commands
\ifdraft
\newcommand{\saurabh}[1]{\marginpar{{\footnotesize\textcolor{orange}{SB:\@ #1}}}\xspace}
\newcommand{\kevin}[1]{\marginpar{{\footnotesize\textcolor{rubine}{KC:\@ #1}}}\xspace}
\newcommand{\mustafa}[1]{\marginpar{{\footnotesize\textcolor{blue}{MA:\@ #1}}}\xspace}
\newcommand{\xing}[1]{\marginpar{{\footnotesize\textcolor{violet}{XG: #1}}}\xspace}
\newcommand{\changes}[2]{\textcolor{red}{CH: (#1) #2}\xspace}
\newcommand{\review}[2]{\marginpar{{#2}}}
\else
\newcommand{\saurabh}[1]{}
\newcommand{\kevin}[1]{}
\newcommand{\mustafa}[1]{}
\newcommand{\xing}[1]{}
\newcommand{\changes}[2]{#2\xspace}
\newcommand{\review}[2]{}
\fi

% Formatting macros
\renewcommand{\paragraph}[1]{
    \iffull
    \medskip\noindent \textbf{#1.\xspace}
    \else
    \noindent \textbf{#1.\xspace}
    \fi
}
% \newcommand{\etal}{\emph{et al.}}
\newcommand{\unbox}{\floatstyle{plain}\restylefloat{figure}}
\newcommand{\rebox}{\floatstyle{boxed}\restylefloat{figure}}
\def\scalefigure{1.0}
\iffull \def\scalefigure{0.7}\fi


==> reviews_sec_revision.tex <==
Reviewer 1's Comments:
======================
Reviewer: 1

Recommendation: Author Should Prepare A Major Revision For A Second Review

Comments:
(1) Thank you to authors for their efforts on revising the paper. It is good to see some improvements of the paper. For example, authors provided brief motivations behind different types of games and now there is a new Figure 2 that provides an overview of research challenges. However, I do not feel that my main comment on contribution of the paper was addressed.

++ MA: Response to (1)
Response: Thanks for such precise summary of our main additions in the previous revision.
++

(2) With a vision piece it would be expected either to offer some exciting perspectives that academics from both camps (Game Theoretic and Distributed Systems Security) would buy into or to support your vision with very clear rigorous review of the relevant literature and its gaps to steer and ignite further interests on the topic. Or, as suggested previously, to discuss the pro’s and con’s of various game-theoretic models.

For example, it is difficult to see the purpose of the “Foundation: Build on Them” section without a come back to these foundation in the further “Challenges ahead” section. The vision needs to offer at least a vague idea on how these games can help with challenges in analytical directions, system directions? And that leads to the next questions: Is chosen differentiation between type of games is the most helpful? Would it work better to flip the approach in the paper and first look at open gaps and questions and then ask what game theoretic models are best suited to answer these questions/fill the gaps and why it would be the most suited ones.

++ MA: Response to (2)
Response: Thanks for such precise comment. We have added a table with the pro’s and con’s of various game-theoretic models as applied to distributed systems security and related research directions in our vision.
++


(3) There need to be more work done on discussions of the models. As an example, the subsection “Static and Complete Information Games” starts with description of a one-stage game, but then when the authors move on to talk about common knowledge and Nash equilibrium the reference is changing to “repeated plays” and essentially, what we know as evolutionary games. Without any transition the reader is dropped from static to dynamic games? There needs to be clarity why in this subsection you start to refer to a different class of games?

++ MA: Response to (3)
Response: Thanks for raising this comment, we have edited this section to capture such transition between different classes of games, and further explained Nash Equilibrium concept, and enhanced transitions between different classes of games that we discuss in this foundations section. We also have related discussions in added Figure (Figure 2).
++ 

(4) In the same sub section the authors come to applications and briefly mention that such games can help to understand botnet defenses. It is surprising not to have any single reference within this section. It would be also great to see what are the findings so far in applying these models – slightly expand on what answers we already have and move beyond “could be useful in understanding system evolution during attack”. Again it feeds into the same issue as I mentioned above – what is the connection between research challenges of Figure 2 and foundation game theoretic models.

++ MA: Response to (4) ++
We have added reference to that section. We added "In particular,
this line of work has provided a comprehensive
game theoretical framework that models the
interaction between the botnet herder and the
defender group (network/computer users). The
Nash equilibrium showed the effectiveness of
available defense strategies and control/strategy
switching thresholds, specified as rates of
infection. This model also showed that integrating
game-theoretical analysis with SIS epidemic
models could be useful in understanding system
behavior during attacks"


Also, we added glue texts to connecting how some challenges we present can be solved (in part) by some of the foundations that we have covered in Foundations section, providing prospective game-theoretic model and systems concept for almost all challenges.



(5) Also the wording “Nash equilibrium has helped understand botnet defenses” does not convey the right sense. It may help to point out why it is relevant within this subsection.

Response: Thanks for raising such a comment. We have clarified such sentence via adding a short explanation why did we mention Nash equilibrium and to further explain such line of work as follows. 
``The Nash equilibrium is the traditional concept capturing efficient solution(s) of complete information games.''

``In particular, this line of work has provided a comprehensive game theoretical framework that models the interaction between
the botnet herder and the defender group (network/computer users). The Nash equilibrium showed the effectiveness of available defense strategies and control/strategy switching thresholds, specified as rates of infection.''



(6) Minor comment. Caption of Figure 1 moved from one extreme to the other. It shall be possible to settle in the middle ground of meaningful but reasonable length caption.

Response: Thanks for raising such concern on updated caption, we agree with your suggestion. We have edited it to be with reasonable length while being meaningful.


## Saurabh's Comments
We need to start the process of collecting the responses to the single reviewer's comments. We can use a macro for indicating additions and chops.

One that I will push back in a note to the EIC is the request for more references --- we are capped by the magazine and through explicit direction by the Editor.
Regarding the other points, here is my high-level take, under the constraint that we have to make the changes space neutral.
1. We add some more text to the vision of where we see this field going. In particular, we speculate on important problems that game theory and distributed systems security can come together to solve. Here you have a chance to put on your creative hat.

+++

Saurabh's additions: 
In the conclusion for the vision using \revadd. 
I also removed some text to make this space neutral, used \choprev. 

+++
2. We add more glue text to connecting how some challenges we present can be solved (in part) by some of the foundations that we have covered. This will not be a complete coverage by any stretch, but some connections will help.

+++

Saurabh's additions: 
I added some material tying to Foundations under: 
(1) Challenges Ahead --> Analytical directions --> Scalability and tractability.
(2) Challenges Ahead --> Integration directions --> Secure distributed applications with partially trusted data sources.
I chopped some material to make this space neutral, from:
Challenges Ahead --> Systems directions --> Designing for security in the tradeoff space.

+++

3. For the game theory discussion, we should add glue text when we move from one type of game to another to justify why the community developed this new formalism.



